Casual Indoor HDR Radiance Capture from Omnidirectional Images

We present PanoHDR-NeRF, a neural representation of the full HDR radiance field of an indoor scene, and a pipeline to capture it casually, without elaborate setups or complex capture protocols. First, a user captures a low dynamic range (LDR) omnidirectional video of the scene by freely waving an off-the-shelf camera around the scene. Then, an LDR2HDR network uplifts the captured LDR frames to HDR, which are used to train a tailored NeRF++ model. The resulting PanoHDR-NeRF can render full HDR images from any location of the scene. Through experiments on a novel test dataset of real scenes with the ground truth HDR radiance captured at locations not seen during training, we show that PanoHDR-NeRF predicts plausible HDR radiance from any scene point. We also show that the predicted radiance can synthesize correct lighting effects, enabling the augmentation of indoor scenes with synthetic objects that are lit correctly. Datasets and code are available at https://lvsn.github.io/PanoHDR-NeRF/.

==> sections/OldIntro.tex <==
%!TEX root = ../main.tex
\section{Introduction}

% \todo{Add Tarko etal somewhere as its the closest thing to what we do, also maybe reword modified nerf++ model as panohdr nerf only }

Capturing the incoming radiance of a given scene is an important step for many augmented reality applications. To accurately measure the radiance, Debevec~\cite{debevec-sig-98} pioneered the use of \emph{image-based lighting} which involves photographing a chrome sphere---called a {\em light probe}---at different exposures and merging them into a single, high dynamic range (HDR) image~\cite{debevec-siggraph-97}. Since then, the process of acquiring HDR light probes has been extended to, for example, the use of wide angle lenses or $360^\circ$ cameras directly. This process is at the heart of the lighting capture necessary to achieve special effects in movies today\footnote{See \url{https://www.fxguide.com/fxfeatured/the-definitive-weta-digital-guide-to-ibl/}.}. 

Because of the close proximity between light sources and objects in the scene, the HDR radiance field of a typical indoor scene varies rapidly: lighting near a window is vastly different than under a table, or close to desk lamp. Therefore, accurately capturing radiance indoors implies moving the apparatus and repeating the operation many times---a process which does not scale. Consequently, approximations such as reprojecting the measured radiance onto a proxy 3D model~\cite{debevec1998efficient} must be used. To simplify the capture process, one could alternatively rely on ``inverse tonemapping'' techniques~\cite{rempel-siggraph-07,reversetone,brown2019} which aim to recover the true dynamic range information from low dynamic range inputs, but this still yields radiance estimates only where images are taken. 

Novel view synthesis of an object or scene from multiple views has garnered attention recently, especially since the emergence of neural radiance fields (NeRF)~\cite{nerf}. In this approach, a set of images are captured, co-registered using structure-from-motion (SfM), and used to train a deep network which learns to predict the color and opacity along any 3D ray using volumetric rendering. Recent flavors of NeRF model unbounded scenes~\cite{nerf++,barron2022mipnerf360}, handle omnidirectional input images~\cite{omni-fish}, and even decompose the scene into intrinsic components~\cite{nerd,nerfactor}, going beyond the original formulation. Unfortunately, most current NeRF-based methods accept low dynamic range (LDR) images as input and do not accurately model the true HDR radiance of indoor environments. Two recent works address this limitation~\cite{hdrnerf,rawnerf}, but neither, as we will demonstrate, is well-suited for modelling the full dynamic range of indoor lighting that frequently spans more than 20 f-stops of dynamic range. 

In this work, we present \methodname: a novel method which enables, for the first time, the casual capture of the full HDR radiance field at any point in an indoor scene. Our method does not require any special equipment nor complicated capture setup. It accepts as input a video sequence captured by freely hand-waving a commercial $360^\circ$ camera around the scene. As output, it produces the HDR radiance at any given location in the scene. To do so, we leverage two deep neural networks: 1) an LDR2HDR model that predicts the HDR radiance from a single LDR panorama captured by the camera and 2) a modified NeRF++ model trained on the predicted HDR outputs of the first network. To evaluate our proposed method, we capture a set of six different indoor scenes, which we augment with a set of ground truth HDR light probes at each scene. Our experiments demonstrate that, despite the simplicity of the capture procedure, \methodname can accurately predict HDR radiance in a variety of challenging conditions. Our approach can render $360^\circ$ HDR light probes, which can then be used to synthesize correct lighting effects, enabling the augmentation of indoor scenes with synthetic objects that are lit correctly. Datasets and code will be released upon publication to spur further research.


% We present PanoHDR-NeRF, a framework to capture the geometric structure and high dynamic range radiance of a typical indoor scene consisting of objects and light sources. Our framework allows generation of new views of the scene as full HDR panoramas. The synthesized panorama is a 2D field of HDR radiance. It can thus be used to manipulate the scene with correct lighting, shading, and shadow effects. The synthesized views, thus, have a high dynamic range and are suitable to be used to model the environment radiance accurately. This allows not only to insert synthetic objects into the scene but also to light them correctly so that shadows and shading appear realistic. Our system only requires a set of LDR panoramas captured by an ordinary camera.


% Omnidirectional images capture the 2D radiance field around a point. 
% High dynamic range (HDR) panoramas are necessary to capture a scene with light sources, windows, etc., if the radiance field has to be used for richer lighting effects in the captured virtual space. 
% However, digital cameras capture images with a limited dynamic range that is insufficient for AR/VR use cases. 



% HDR images can be obtained by merging multiple LDR images at different exposures~\cite{debevec-siggraph-97} but this leads to ghosting effects and requires a specialized setup. 

% Single Image HDR reconstruction aims to recover information from a single low dynamic range (LDR) image by filling the missing information in under/over exposed regions. 

% Liu \etal~\cite{hallu} explicitly model the inverse functions of LDR image formation for reconstructing HDR images. However their Hallucination Net cannot recover bright light sources necessary for indoor scenes. 

% Yu \etal~\cite{lanet} proposes a luminance attention network (LANet) that learns an attention map for under/over exposed regions. 

% These have to be adapted to panorama images as input and to generate very high dynamic ranges for AR/VR applications.

% Tarko \etal~\cite{brown2019} use recovered HDR panoramas to perform virtual object insertion with correct lighting. They do it for captured frames and cannot alter the view points. 

% Neural radiance fields~\cite{nerf} are effective in novel view synthesis but typically use perspective, LDR images. OmniNeRF extends the framework to LDR panoramas using a pair of color and aligned depth panoramas~\cite{omninerf}. While panorama capture is an easy operation, getting aligned depth panoramas requires special equipment. Besides, they can perform synthesis only for views lying on a straight line.

% We need to generate new views as HDR panoramas to solve the problem. HDRNeRF~\cite{huang2021hdr} estimates the HDR radiance fields from a set of LDR images at different exposures. However, capturing LDR images at different exposures requires an elaborate setup and can give way to ghosting artifacts. NeRF in the Dark~\cite{mildenhall2021nerf} uses raw images to train NeRF and captures 14 or 16 bit radiance values. Synthesizing a panorama with normally lit regions and visible light sources needs higher dynamic range than what these methods provide.

% We present PanoHDR-NeRF, a framework to capture the geometric structure and high dynamic range radiance of a typical indoor scene consisting of objects and light sources. Our framework allows generation of new views of the scene as full HDR panoramas. The synthesized panorama is a 2D field of HDR radiance. It can thus be used to manipulate the scene with correct lighting, shading, and shadow effects. The synthesized views, thus, have a high dynamic range and are suitable to be used to model the environment radiance accurately. This allows not only to insert synthetic objects into the scene but also to light them correctly so that shadows and shading appear realistic. Our system only requires a set of LDR panoramas captured by an ordinary camera.





% % why is capturing radiance important
% Capturing the incoming radiance of a given scene is an important step for ... To accurately capture the radiance at a given point in the scene, Debevec~\cite{debevec-sig-98} pioneered the use of \emph{image-based lighting} and suggested to capture several exposures of a chrome sphere---dubbed a ``light probe''---at a given location, and fuse the resulting images into a single, high dynamic range (HDR) image~\cite{debevec-siggraph-97}. Alternatively, HDR light probes can also be captured with cameras with wide-angle lenses, or $360^\circ$ cameras directly. This process is still at the heart of the lighting capture process necessary to achieve special effects in movies today\footnote{See \url{https://www.fxguide.com/fxfeatured/the-definitive-weta-digital-guide-to-ibl/}.}.

% % how to do it? -- limitations: tedious, must be performed everywhere
% The main limitation of this technique is that capturing a single light probe is tedious: because several exposures must be captured and fused, the camera must be held still with a tripod. In order to more densely capture the indoor radiance of a scene, it is necessary to physically move this setup and repeat the operation as many times as needed to cover the desired volume. Naturally, this process does not scale. 

% % leverage view interpolation techniques? 
% In this paper, we propose to leverage novel view interpolation techniques based on ... to learn to reconstruct the radiance of an indoor scene given a video of the scene captured using a handheld commercial $360^\circ$ camera. A photographer can simpy hand-wave the camera around the scene in a casual manner to capture several views of that scene. Then, we train a NeRF model (more specifically the NeRF++ variant~\cite{nerf++}) which learns to predict the appearance of the scene from any viewpoint. 

% Unfortunately, neural radiance field methods are limited by the dynamic range of the input images on which they are trained. To alleviate this, recent approaches have proposed to adapt NeRF models to accept as input sequences captured at alternating exposures~\cite{huang2021hdr}, or RAW images~\cite{mildenhall2021nerf} (which may have up to 14- and even 16-bits effective dynamic range). However, due to the presence of very bright light sources, the full dynamic range of indoor scenes may exceed what can be captured with these techniques. Therefore, we propose to combine spherical NeRF models



% Capturing the structure and complete radiance of a scene is important to provide virtual and augmented reality experiences around it. The captured scene can be synthesized from arbitrary viewpoints while also manipulating it with correct lighting, shading, and shadow effects. Ability to do that will help close the gap between real scenes and their virtual/augmented versions.

% Expensive setups and structure from motion techniques have been replaced with variants of NeRF~\cite{nerf} recently. Capturing the scene radiance for accurate synthesis of lighting effects, however, has not had similar success. Expensive setups and lightprobes are not practical and radiance capture using them is tedious.


==> sections/background.tex <==
%!TEX root = ../main.tex
%\section{Background}
\paragraph{Background}

% \subsection{Neural Radiance Fields}
%  NeRF~\cite{nerf} represents a scene as an implicit continuous 5D function that maps every points with the position $(x,y,z)$ and the viewing direction $(\theta,\phi)$ to the their corresponding transmitted radiance \textbf{c} and volume density $\sigma$. NeRF predicts the color $\hat{C}$ of any ray $\textbf{r}$ passing through the scene by sampling $s$ points along the ray between the $t_\mathrm{near}$ and $t_\mathrm{far}$ and combining them as $\hat{C}(\mathbf{r}) = \int_{t_\mathrm{near}}^{t_\mathrm{far}}T(s)\sigma(\textbf{r}(s))\textbf{c}(\textbf{r}(s),\textbf{d})ds$, where $\textbf{d}$ is the viewing direction and $T(s) = \exp\left(-\int_{t_\mathrm{near}}^{t_\mathrm{far}}\sigma(\textbf{r}(p))dp\right)$ is the accumulated transmittance along the ray. To learn the scene, NeRF uses the loss between predicted color $\hat{C}$ and ground truth $C$ as $\ell_\mathrm{nerf} =  \sum_{r \in\mathcal{R}(\textbf{P})} \|\hat{C}(\textbf{r}) - C(\textbf{r})\|^2$, where $\mathcal{R}(\textbf{P})$ is the set of camera rays at point $\textbf{P}$. %NeRF optimizes two models: coarse and fine. The densities procured from the coarse model guide the sampling for the fine model. In addition, NeRF applies positional encoding that maps the input to a higher dimension and enables the network to learn higher frequencies of data.
  
% \subsection{Unbounded Neural Radiance Fields}
% \label{sec:nerpp}
% Although NeRF is able to encode bounded scenes, it struggles to accurately represent indoor scenes with large scene coordinates and is unable to reconstruct the scene. NeRF++~\cite{nerf++} proposes dividing the scene space into two volumes: an inner sphere (foreground) modelling the volume that bounds all camera locations; and an outer volume (background) representing anything farther away. The parameterization for the foreground is the same as the original NeRF. For the background, a 3D point $(x,y,z)$ is parameterized by the quadruple $(x',y',z',1/r)$ where $(x',y',z')$ is a unit vector representing a direction on the sphere and $0<1/r<1$ is the inverse radius (disparity) along this direction specifying the point $r\cdot(x',y',z')$. %NeRF++ trains separate models for the foreground and background and combine their results. 
% We use NeRF++ as the base architecture for our approach.

%\subsection{Unbounded Neural Radiance Fields}
\label{nerfpp}
NeRF~\cite{nerf} represents a scene as an implicit continous 5D function that maps a 3D point with position $(x,y,z)$ and viewing direction $(\theta,\phi)$ to their corresponding transmitted radiance \textbf{$c$} and volume density \textbf{$\sigma$}. For a given ray \textbf{$r$} passing through scene, NeRF predicts $\hat{C}$ by sampling $s$ points along the ray and predicting \textbf{$c$} and \textbf{$\sigma$} and combining them with classic volumetric rendering techniques. Although it is able to encode bounded scenes, it struggles to reconstruct unbounded indoor scenes. NeRF++~\cite{nerf++} divides the screen space into an inner sphere (foreground) volume that models all camera locations; and an outer (background) volume representing anything farther away. Foreground is parameterized same as NeRF. A 3D point $(x,y,z)$ in the background is parameterized by the quadruple $(x',y',z',1/r)$ where $(x',y',z')$ is a unit vector representing a direction on the sphere and $0<1/r<1$ is the inverse radius (disparity) along this direction specifying the point $r\cdot(x',y',z')$. NeRF++ trains separate models for the foreground and background and combine their results. 



==> sections/copyRelWork.tex <==
%!TEX root = ../main.tex
\section{Related work}

% Here, we focus on inverse tonemapping, novel view synthesis and neural radiance fields as the most related works to ours.

\paragraph{Inverse tonemapping} The extrapolation of high dynamic range data from low dynamic range input, a process known as inverse tonemapping, aims to recover missing information in the over- and under-saturated areas of an LDR image. While earlier methods~\cite{rempel-siggraph-07} mostly relied on heuristics, deep learning has been employed for this task since 2017~\cite{reversetone,rendering}. Several network architectures have been proposed, such as a 2D encoder and 3D decoder with skip connections to generate bracketed LDR image stacks (up exposed and down exposed)~\cite{reversetone}, an encoder-decoder to reconstruct the HDR image directly~\cite{hdrnet}, or a multiscale autoencoder architecture to learn multilevel features from LDR image which are merged to reconstruct HDR images~\cite{expandnet}. Lee \etal~\cite{deepchain} also generate LDR stacks but with a two-branch network. DeepHDR~\cite{deephdr} show that using the same CNN filters for well-exposed and saturated pixels is sub-optimal, and propose to mask out the saturated areas thus reducing the contribution of features from these areas. 

Another approach, dubbed HallucinationNet~\cite{hallu}, proposes to individually model the main components of the imaging pipeline, namely: dynamic range clipping, camera response function, and quantization. 
%Tailored DNN models are then trained to sequentially learn the three reverse steps, and finally jointly fine-tuned in an end-to-end manner. 
LANet~\cite{lanet} introduces a multi-task network with a luminance attention and HDR reconstruction streams. 
%The former creates a spatially-weighted attention map of overexposed regions which is utilized to reconstruct HDR images faithfully. 
In this work, we rely on the LANet architecture, which we also augment with an additional rendering loss. We show that this combination outperforms alternatives at predicting the high dynamic range radiance in indoor environments. 

% Endo \etal~\cite{reversetone} proposed a framework with a 2D encoder and 3D decoder with skip connections to generate bracketed LDR image stacks (up exposed and down exposed) from an HDR image using the camera response function (CRF) database. 
% Lee \etal~\cite{deepchain} generated LDR stacks with a two branch network. Three up and down exposed LDR stacks are generated sequentially and merged to generate an HDR image. Multi exposure stacks in both are generated using GANs which introduce their own biases and hence limit the capability of such models.
% HDRCNN~\cite{hdrnet} on the other hand, leverages an encoder decoder based architecture to reconstruct the HDR image from a single LDR image. 
% ExpandNet~\cite{expandnet} utilizes a multiscale autoencoder architecture to learn multilevel features from LDR image which are merged to reconstruct HDR images. 


\paragraph{Novel view synthesis} Classical methods reconstruct an explicit 3D model to represent the scene~\cite{debevec1998efficient,GortlerGSC96,HedmanRDB16}. Methods such as~\cite{hedman18siggraph,meshry19cvpr,dnr} utilize off-the-shelf structure from motion (SfM) techniques to generate a coarse, imperfect geometry of the scene, and train neural rendering approaches to render photorealistic images at novel views. Another approach suggests breaking the scene into multiplane image (MPI)~\cite{flynn19cvpr,stereo18tog,llff} representation and render novel views through blending. Sitzmann et al.~\cite{sitzmann19cvpr} learn a voxel-based volumetric representation of the scene using gated recurrent units (GRUs)~\cite{DBLP:conf/emnlp/ChoMGBBSB14}. \cite{Riegler2020FVS} performs view synthesis by mapping the encoded features from the source images into the target view and blending them via a neural network. \cite{Riegler2021StableVS} does the same by mapping encoded image feature vectors onto the reconstructed geometry and aggregating these features for a novel view.

Attempts for novel view synthesis from omnidirectional images have been fairly limited so far. Huang \etal~\cite{huangpano} attempt to reconstruct a point cloud from input $360^\circ$ video to achieve real time 6-DoF video playback on a VR device. Serrano \etal~\cite{serrano} design a layered scene representation which facilitates parallax and real tome playback of $360^\circ$ video. Lin \etal~\cite{linpano} and Attal \etal~\cite{attalpano} present multidepth panorama (MDP) and multi-sphere images to conduct 6 DoF renderings. However, this does not accommodate free viewpoint synthesis and requires an elaborate setup. Xu \etal~\cite{xupano} estimate the entire indoor scene from a single image using CNN based network. However, they require room layout priors and depth which are time consuming and challenging to obtain for real world scenes. 

\paragraph{Neural radiance fields}

% Implicit scene representations are a new class of methods which leverage multi-layer perceptrons (MLP) to encode a scene to perform novel view synthesis. 
Neural Radiance Fields (NeRF)~\cite{nerf} learn an implicit scene representation with a multi-layer perceptron (MLP) that receives viewing positions and directions as input and predicts the RGB colour and opacity as output. 
%Pixel colors are rendered by combining the outputs of the network using traditional volume rendering~\cite{ray_tracing84}. 
The original NeRF formulation was later extended in several ways---we only list the most relevant to our work.
First, NeRF++~\cite{nerf++}, which we leverage, models an unbounded scene by splitting it into foreground/background, and by learning each separately. Similarly, Mega-NeRF~\cite{meganerf} divides the scene into smaller sections, and Block-NeRF~\cite{blocknerf} splits city-scale scenes into blocks, trains a NeRF for each block, and combines the results. 
% Since we are modelling indoor rooms which are of a smaller scale, a foreground-background parameterization is more than sufficient. 
Second, sampling was revisited in Mip-NeRF~\cite{mipnerf,barron2022mipnerf360}, which replaces rays with anti-aliased conical frustums.

Third, and of particular relevance to our work, the ability to deal with high dynamic range data has been explored in two works. NeRF in the dark~\cite{rawnerf} train directly on linear RAW images, which contain higher effective dynamic range than typical 8-bit cameras (up to 14--16 bits for high quality DSLRs. We show that this higher dynamic range is still not high enough to accurately capture radiance in most indoor environments. Huang \etal~\cite{hdrnerf} learns the HDR radiance field from a set of LDR images captured at alternating exposures, which needs a more elaborate capture setup. In contrast, our method accurately models the full dynamic range from a single input video. 

Finally, panoramic images have been explored in \cite{omninerf,omni++}, who present a method for synthesizing panoramas from a single omnidirectional input. Unlike ours, these works require depth as input, and novel views are only rendered on a straight line. \cite{omni-fish} synthesizes novel fish-eye projection images and like our method, incorporates spherical sampling to improve the quality of results.

% Image formation is a complex process of how light interacts with materials and camera to form an image on the camera's sensor. Then the final image is created by applying tonemapping to be visually pleasing for the viewer. NeRF bakes these complex interactions by assuming the scene as a low dynamic range (LDR) radiance field. LDR capturing cannot truly represent the light intensities, which is problematic for realistic image-based lighting and virtual object insertion.

\input{sections/figures/method-fig}

\paragraph{HDR scene capture}

Zhang \etal~\cite{zhang2016emptying} leverage an RGBD scan of an indoor scene and estimated various scene parameters including HDR radiances over scene geometry. Similarly, Walton \etal~\cite{waltondynamic} combine a depth sensor with a fisheye camera in a SLAM-based approach to recover geometry and lighting. Tarko \etal~\cite{brown2019} takes an omnidirectional video as input and uses inverse tone mapping~\cite{reversetone} to convert the video to HDR. Yang \etal~\cite{yangneural} learn a background and objects as separate NeRF models, then combine them together with a captured panoramic image into a single scene. In contrast to these works, we focus on simultaneously learning HDR and viewpoint synthesis. 

% Song \etal~\cite{songneural} attempted to estimate the HDR light intensity at a given point in a LDR image. Their objective was to estimate HDR lighting for all points and use that to relight virtual objects correctly. However, they cannot perform novel view synthesis. 


==> sections/data.tex <==
%!TEX root = ../main.tex
\section{Data}
\subsection{Radiance Capture}
\label{sec:dataset}


\subsection{PanoHDR-NeRF}
For each scene, we casually capture a set of LDR panoramas using a commercial $360^\circ$ camera to train the PanoHDR NeRF. For this, we first fix the camera (we use a Ricoh Theta Z1 model) on a portable tripod. We then capture a $360^\circ$ video while waving the camera around the scene to cover the entire volume as much as possible for a few minutes (typically 3--5 minutes for the scenes used in the experiments). Approximately 200 frames are then extracted from the video at even intervals. Since this method implies that a photographer will be waving the camera around, we use Mask R-CNN~\cite{he2017mask} to produce segmentation masks for humans in the scene.

We also capture a set of 10 HDR panoramas per scene to use as ground truth for evaluation. To obtain these, we set the camera on a tripod at certain locations in the scene (we capture approximately 10 locations per scene). We use exposure bracketing mode to capture 11 exposures that are subsequently fused to HDR using the PTGui Pro commercial software. We also capture a short video with the same camera parameters as the first one at the same location as the HDR. We then extract a single frame from the video, allowing us to have an LDR image at the exact same location as its HDR counterpart.

Ultimately, we linearize the frames extracted from the videos. So, for each scene, we have about 10 HDR panoramas with their LDR counterparts, and about 200 LDR images taken everywhere around the scene, with corresponding segmentation masks. We collect 6 such datasets as shown in fig.~\ref{fig:dataset_mosaic}.

==> sections/figures/create_hdr.tex <==
\begin{figure}
    \centering
    \footnotesize
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccc} 
    %     \hline
    %   LDR &  LANet Render & Sensor FT & GT\\ \hline
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012879.JPG} &
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012880.JPG} &
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012881.JPG} \\
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012882.JPG} &
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012883.JPG} &
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012884.JPG} \\
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012885.JPG} &
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012886.JPG} &
       \includegraphics[width=0.32\linewidth]{figures/datasets_sample/exposures/R0012887.JPG} \\
    \end{tabular}
    \caption{We capture multiple panorams at different exposures which are ultimately combined to produce HDR images.}
    \label{fig:hdr_cap}
\end{figure}

==> sections/figures/rawnerf_comp.tex <==
%!TEX root = ../../main.tex


\begin{figure*}[b]
\centering
\setlength{\tabcolsep}{1pt}
\footnotesize
\begin{tabular}{cccc}
& Original exposure & Divided by 8 & Divided by 32 \\
\rotatebox[origin=c]{90}{RAW} &
\includegraphics[width=0.315\linewidth,valign=m]{figures/raw_nerf_comp/raw_0.png} &
\includegraphics[width=0.315\linewidth,valign=m]{figures/raw_nerf_comp/raw_3.png} &
\includegraphics[width=0.315\linewidth,valign=m]{figures/raw_nerf_comp/raw_5.png} \\*[2.2em]
\rotatebox[origin=c]{90}{Ours} &
\includegraphics[width=0.315\linewidth,valign=m]{figures/raw_nerf_comp/ours_0.png} &
\includegraphics[width=0.315\linewidth,valign=m]{figures/raw_nerf_comp/ours_3_signs.png} &
\includegraphics[width=0.315\linewidth,valign=m]{figures/raw_nerf_comp/ours_5_signs.png}
\end{tabular}
\caption{Comparing the dynamic range of a single RAW image (top, as used in \cite{rawnerf}) with the output of our LDR2HDR network (bottom) at different exposures. A single RAW image is insufficient to capture the full dynamic range of typical indoor scenes. }
\label{fig:rawnerf-comp}
\end{figure*}


==> sections/figures/test.tex <==
%!TEX root = ../../main.tex
\begin{figure*}[t]
    \centering
    % \footnotesize
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{cccc} 
        & NeRF++ & PanoHDR-NeRF & HDR GT \\ 
        % \multirow{2}{*}{\rotatebox[origin=c]{90}{Spotlights}} & 
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/ldr_old_class_spot.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_old_class_spot.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/ft_old_class_spot.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/gt_old_class_spot.jpeg} \\
        % & 
        \rotatebox[origin=c]{90}{Spotlights} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_ldr_nerf_old_class_spot.jpeg} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_ldr2hdr_nerf_old_class_spot.jpeg} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_gt_old_class_spot.jpeg} \\*[3em]
        
        \rotatebox[origin=c]{90}{Stairway} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_ldr_nerf_stairway.jpeg} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_ldr2hdr_nerf_stairway.jpeg} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_gt_stairway.jpeg} \\*[3em]
        
        \rotatebox[origin=c]{90}{Chess room} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_ldr_nerf_chess_room.jpeg} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_ldr2hdr_nerf_chess_room.jpeg} &
        \includegraphics[width=0.33\linewidth,valign=m]{figures/nerf/render_gt_chess_room.jpeg} \\*[3em]
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_gt_old_class_spot.jpeg} \\*[3em]
        
        % \multirow{2}{*}{\rotatebox[origin=c]{90}{Stairway}} & 
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/ldr_stairway.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_stairway.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/ft_stairway.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/gt_stairway.jpeg} \\
        % &
        % \rotatebox[origin=c]{90}{Stairway} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_ldr_stairway.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_render_stairway.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_ft_stairway.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_gt_stairway.jpeg} \\*[3em]
        
        % % \multirow{2}{*}{\rotatebox[origin=c]{90}{Small classroom}} & 
        % % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/ldr_small_class.jpeg} &
        % % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_small_class.jpeg} &
        % % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/ft_small_class.jpeg} & 
        % % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/gt_small_class.jpeg} \\
        % % & 
        % \rotatebox[origin=c]{90}{Small classrm} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_ldr_small_class.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_render_small_class.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_ft_small_class.jpeg} &
        % \includegraphics[width=0.24\linewidth,valign=m]{figures/render/render_gt_small_class.jpeg} \\
    \end{tabular}
    \caption{}
    \Description{Qualitative comparison.}
    \label{fig:ldr2hdr-qual}
\end{figure*}

==> sections/tables.tex <==
% \begin{table*}[ht]
% \caption{Quantatitive analysis between different strategies across scenes}
% \centering
% \label{tab:quant-scenes}
%   \begin{tabular}{lSSSSSSSSS}
%     \toprule
%     \multirow{3}{*}{Dataset} &
%       \multicolumn{3}{c}{LANet Render} &
%       \multicolumn{3}{c}{Sensor FT} &
%       \multicolumn{3}{c}{1HDR FT} \\
%       & {PU-PSNR$\uparrow$} & {PU-SSIM$\uparrow$} &  {HDR-VDP3$\uparrow$} & {PU-PSNR$\uparrow$} & {PU-SSIM$\uparrow$} &  {HDR-VDP3$\uparrow$} & {PU-PSNR$\uparrow$} & {PU-SSIM$\uparrow$} &  {HDR-VDP3$\uparrow$} \\
%       \midrule
%     chess room & 33.994 & 0.954 & 8.234 & 36.995 & 0.956 & 8.492 & 37.561 & 0.955 & 8.521 \\
%     cafeteria & 26.664 & 0.941 & 6.418 & 28.499 & 0.936 & 7.164 & 29.621 & 0.943 & 7.444 \\
%     kitchen & 28.934 & 0.921 & 6.655 & 29.612 & 0.901 & 7.214 & 30.797 & 0.910 & 7.286 \\
%     living room & 31.099 & 0.917 & 7.222 & 32.354 & 0.919 & 7.511 & 32.822 & 0.921 & 7.681 \\
%     old class spot & 25.118 & 0.932 & 6.097 & 28.966 & 0.929 & 7.667 & 29.694 & 0.930 & 7.667 \\
%     old class neon & 32.125 & 0.920 & 7.592 & 32.594 & 0.918 & 8.135 & 32.934 & 0.915 & 8.165 \\
%     guest room & 34.205 & 0.917 & 8.003 & 34.923 & 0.914 & 8.129 & 35.022 & 0.915 & 8.160 \\
%     attic & 38.049 & 0.940 & 7.793 & 36.972 & 0.935 & 7.810 & 36.759 & 0.946 & 7.776 \\
%     small class & 34.095 & 0.955 & 8.267 & 35.465 & 0.952 & 8.678 & 38.116 & 0.957 & 8.732 \\
%     stairway & 33.297 & 0.960 & 8.016 & 33.685 & 0.957 & 8.489 & 34.385 & 0.959 & 8.366 \\
%     music room & 37.712 & 0.908 & 7.636 & 36.435 & 0.906 & 7.638 & 38.320 & 0.942 & 7.706 \\
%     \hline
%     overall & 32.299 & 0.933 & 7.448 & 34.318 & 0.929 & 7.902 & 35.184 & 0.935 & 8.015\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% \begin{table*}[ht]
% \caption{Quantatitive analysis between different strategies across scenes}
% \centering
% \label{tab:quant-scenes}
%   \begin{tabular}{lSSSSSSSSS}
%     \toprule
%     \multirow{3}{*}{Dataset} &
%       \multicolumn{3}{c}{LANet Render} &
%       \multicolumn{3}{c}{Sensor FT} &
%       \multicolumn{3}{c}{1HDR FT} \\
%       & {PU-PSNR$\uparrow$} & {R-MSE$\downarrow$} &  {HDR-VDP3$\uparrow$} & {PU-PSNR$\uparrow$} & {R-MSE$\downarrow$} &  {HDR-VDP3$\uparrow$} & {PU-PSNR$\uparrow$} & {R-MSE$\downarrow$} &  {HDR-VDP3$\uparrow$} \\
%       \midrule
%     chess room & 33.994 & 0.048 & 8.234 & 36.995 & 0.005 & 8.492 & 37.561 & 0.008 & 8.521 \\
%     cafeteria & 26.664 & 5.268 & 6.418 & 28.499 & 4.061 & 7.164 & 29.621 & 2.284 & 7.444 \\
%     kitchen & 28.934 & 14.454 & 6.655 & 29.612 & 13.985 & 7.214 & 30.797 & 14.084 & 7.286 \\
%     living room & 31.099 & 0.246 & 7.222 & 32.354 & 0.072 & 7.511 & 32.822 & 0.059 & 7.681 \\
%     old class spot & 25.118 & 3.438 & 6.097 & 28.966 & 0.877 & 7.667 & 29.694 & 1.575 & 7.667 \\
%     old class neon & 32.125 & 0.340 & 7.592 & 32.594 & 0.262 & 8.135 & 32.934 & 0.207 & 8.165 \\
%     guest room & 34.205 & 2.808 & 8.003 & 34.923 & 2.468 & 8.129 & 35.022 & 2.212 & 8.160 \\
%     attic & 38.049 & 0.458 & 7.793 & 36.972 & 0.276 & 7.810 & 36.759 & 0.269 & 7.776 \\
%     small class & 34.095 & 1.889 & 8.267 & 35.465 & 0.221 & 8.678 & 38.116 & 0.035 & 8.732 \\
%     stairway & 33.297 & 0.213 & 8.016 & 33.685 & 0.019 & 8.489 & 34.385 & 0.045 & 8.366 \\
%     music room & 37.712 & 0.049 & 7.636 & 36.435 & 0.040 & 7.638 & 38.320 & 0.011 & 7.706 \\
%     \hline
%     overall & 32.299 & 2.651 & 7.448 & 34.318 & 2.025 & 7.902 & 35.184 & 1.889 & 8.015\\
%     \bottomrule
%   \end{tabular}
% \end{table*}



% \begin{table*}[ht]
% \caption{Quantatitive analysis between different strategies across scenes}
% \setlength{\tabcolsep}{2pt}
% \centering
% \label{tab:quant-scenes}
%   \begin{tabular}{lSSSSSSSSS}
%     \toprule
%     \multirow{3}{*}{Dataset} &
%       \multicolumn{3}{c}{LDR} &
%       \multicolumn{3}{c}{LANet Render} &
%       \multicolumn{3}{c}{Sensor FT} \\
%       & {PU-PSNR$\uparrow$} & {PU-SSIM$\uparrow$} &  {HDR-VDP3$\uparrow$} & {PU-PSNR$\uparrow$} & {PU-SSIM$\uparrow$} &  {HDR-VDP3$\uparrow$} & {PU-PSNR$\uparrow$} & {PU-SSIM$\uparrow$} &  {HDR-VDP3$\uparrow$} \\
%       \midrule
%     chess room & 31.659 & 0.953 & 8.067 & 33.994 & 0.954 & 8.234  & 36.995 & 0.956 & 8.492 \\
%     cafeteria & 25.299 & 0.940 & 6.098 & 26.664 & 0.941 & 6.418 & 28.499 & 0.936 & 7.164 \\
%     kitchen & 27.838 & 0.921 & 6.411 & 28.934 & 0.921 & 6.655 & 29.612 & 0.901 & 7.214 \\
%     living room & 29.925 & 0.916 & 7.208 & 31.099 & 0.917 & 7.222 & 32.354 & 0.919 & 7.511 \\
%     old class spot & 23.939 & 0.932 & 6.001 & 25.118 & 0.932 & 6.097 & 28.966 & 0.929 & 7.667 \\
%     old class neon & 30.657 & 0.920 & 7.429 & 32.125 & 0.920 & 7.592 & 32.594 & 0.918 & 8.135 \\
%     guest room & 33.073 & 0.917 & 7.875 & 34.205 & 0.917 & 8.003 & 34.923 & 0.914 & 8.129 \\
%     attic & 37.988 & 0.940 & 7.690 & 38.049 & 0.940 & 7.793 & 36.972 & 0.935 & 7.810 \\
%     small class & 32.353 & 0.953 & 8.018 & 34.095 & 0.955 & 8.267 & 35.465 & 0.952 & 8.678 \\
%     stairway & 31.964 & 0.960 & 7.881 & 33.297 & 0.960 & 8.016 & 33.685 & 0.957 & 8.489 \\
%     music room & 36.584 & 0.904 & 7.533 & 37.712 & 0.908 & 7.636 & 36.435 & 0.906 & 7.638 \\
%     \hline
%     overall & 31.025 & 0.932 & 7.293 & 32.299 & 0.933 & 7.448 & 34.318 & 0.929 & 7.902\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

==> sections/tables/log_loss.tex <==
%!TEX root = ../../main.tex
\begin{table}[th]
\caption{Quantitative comparison between loss used for training PanoHDR NeRF across captured scenes.}
\setlength{\tabcolsep}{2pt}
\centering
  \label{tab:log_loss}
  \begin{tabular}{lcccccc}
    \toprule
    % \multirow{3}{*}{Dataset} &
    & \multicolumn{3}{c}{Log space} &
    \multicolumn{3}{c}{Linear space} \\
    & PU- & \multirow{2}{*}{RMSE$_\downarrow$} & HDR- & PU- & \multirow{2}{*}{RMSE$_\downarrow$} & HDR- \\
    & PSNR$_\uparrow$ &  & VDP3$_\uparrow$ & PSNR$_\uparrow$ &  & VDP3$_\uparrow$ \\
    % & PU-PSNR$_\uparrow$ & R-MSE$_\downarrow$ & HDR-VDP3$_\uparrow$ & {PU-PSNR$_\uparrow$} & {R-MSE$_\downarrow$} &  {HDR-VDP3$_\uparrow$} \\
    \midrule
    Chess room & 35.941 & 0.012 & 7.941 & 35.152 & 0.011 &  7.929 \\
    Stairway & 32.169 & 0.056 & 7.889 & 31.810 & 0.055 & 7.667  \\
    Cafeteria & 27.029 & 4.179 & 6.395 & 24.139 & 4.376 & 6.125  \\
    Spotlights & 27.657 & 0.431 & 7.456 & 26.719 & 0.909 & 7.288 \\
    Dark class. & 29.687 & 1.509 & 7.524 & 28.431 & 1.367 & 7.635  \\
    Small class. & 36.687 & 0.054 & 7.709 & 36.829 & 0.043 & 7.861  \\
    \midrule
    Overall & 31.528 & 1.038 & 7.485 & 29.725 & 1.071 & 7.388 \\
    \bottomrule
  \end{tabular}
\end{table}

==> sections/tables/order.tex <==
%!TEX root = ../../main.tex
\begin{table}[th]

\setlength{\tabcolsep}{2pt}
\centering
\label{tab:order}
  \begin{tabular}{lcccccc}
    \toprule
    % \multirow{3}{*}{Dataset} &
    & 
    \multicolumn{3}{c}{LDR2HDR $\rightarrow$ NeRF} &
    \multicolumn{3}{c}{NeRF $\rightarrow$ LDR2HDR} \\
    % & PU-PSNR$_\uparrow$ & RMSE$_\downarrow$ & HDR-VDP3$_\uparrow$ & PU-PSNR$_\uparrow$ & RMSE$_\downarrow$ & HDR-VDP3$_\uparrow$ \\
    & PU- & \multirow{2}{*}{RMSE$_\downarrow$} & HDR- & PU- & \multirow{2}{*}{RMSE$_\downarrow$} & HDR- \\
    & PSNR$_\uparrow$ &  & VDP3$_\uparrow$ & PSNR$_\uparrow$ &  & VDP3$_\uparrow$ \\
    \midrule
    Chess room & 35.941 & 0.012 & 7.941 & 35.991 & 0.006 &  8.292 \\
    Stairway & 32.169 & 0.056 & 7.889 & 32.707 & 0.055 & 7.740  \\
    Cafeteria & 27.029 & 4.179 & 6.395 & 26.537 & 5.298 & 6.325 \\
    Spotlights & 27.657 & 0.431 & 7.456 & 27.324 & 1.619 & 7.068 \\
    Dark class. & 29.687 & 1.509 & 7.524 & 29.819 & 0.621 & 7.738  \\
    Small class. & 36.687 & 0.054 & 7.709 & 38.529 & 0.006 & 8.059  \\
    \midrule
    Overall & 31.528 & 1.038 & 7.485 & 31.650 & 1.301 & 7.523 \\
    \bottomrule
  \end{tabular}
  \caption{Quantitative comparison between order of LDR2HDR network and PanoNeRF across captured scenes.}
\end{table}
